Behind Every Domain There is a Shift: Adapting Distortion-aware Vision Transformers for Panoramic Semantic Segmentation

In this paper, we address panoramic semantic segmentation which is under-explored due to two critical challenges: (1) image distortions and object deformations on panoramas; (2) lack of semantic annotations in the 360{\deg} imagery. To tackle these problems, first, we propose the upgraded Transformer for Panoramic Semantic Segmentation, i.e., Trans4PASS+, equipped with Deformable Patch Embedding (DPE) and Deformable MLP (DMLPv2) modules for handling object deformations and image distortions whenever (before or after adaptation) and wherever (shallow or deep levels). Second, we enhance the Mutual Prototypical Adaptation (MPA) strategy via pseudo-label rectification for unsupervised domain adaptive panoramic segmentation. Third, aside from Pinhole-to-Panoramic (Pin2Pan) adaptation, we create a new dataset (SynPASS) with 9,080 panoramic images, facilitating Synthetic-to-Real (Syn2Real) adaptation scheme in 360{\deg} imagery. Extensive experiments are conducted, which cover indoor and outdoor scenarios, and each of them is investigated with Pin2Pan and Syn2Real regimens. Trans4PASS+ achieves state-of-the-art performances on four domain adaptive panoramic semantic segmentation benchmarks. Code is available at https://github.com/jamycheung/Trans4PASS.

==> tables/tab7_structure_ablation.tex <==

\begin{table}[!t]
\centering
\caption{\small \textbf{\revised{Trans4PASS+ structural analysis.}} 
$\textbf{*}$ and $\dagger$ denote DPT~\cite{chen2021dpt} and our DPE, while $\ddag$ is trained with OHEM. ``\textbf{\#P}'' is short for \#Parameters in millions. \textbf{CX}: Channel Mixer, \textbf{PX}: Pooling Mixer with 3${\times}$3). Models are trained on Cityscapes~(\textbf{CS})~$@$~512${\times}$512 and tested on DensePASS~(\textbf{DP})~$@$~2048${\times}$400.}
\resizebox{\columnwidth}{!}{
\setlength\tabcolsep{2.0pt}
\begin{tabular}{@{}l@{}ll@{}|rccl@{}}
    \toprule
    \textbf{Network} & \textbf{Encoder} & \textbf{Decoder} & \scriptsize{\textbf{GFLOPs}} & \textbf{\#P} & \textbf{CS} & \textbf{DP}\\ 
    \midrule     \midrule    
    \multicolumn{7}{@{}p{\columnwidth}@{}}{\textit{\textbf{(1) Compare PEs and MLPs:}}} \\ \midrule
    Trans4PASS & MiT-B1${\textbf{*}}$ & DMLPv1+DPT~\cite{chen2021dpt} & 13.11 & 13.10 & 69.48 & 36.50 \\
    Trans4PASS & MiT-B1$\dagger$ & CycleMLP~\cite{cyclemlp}+DPE & 9.83 & 13.60 & 73.49 & 40.16 \\
    Trans4PASS & MiT-B1$\dagger$ & ASMLP~\cite{asmlp}+DPE & 13.40 & 14.19 & 73.65 & 42.05 \\ 
    \rowcolor{gray!15} Trans4PASS & MiT-B1$\dagger$ & DMLPv1+DPE & 12.02 & 13.93 & 72.49 & 45.89~\gbf{+9.39} \\ \midrule[1pt]
    \multicolumn{7}{@{}p{\columnwidth}@{}}{\textit{\textbf{(2) Compare encoders and decoders: }}} \\ \midrule
    PVT~\cite{pvt} & PVT-T & FPN   & 11.17 & 12.76 & 71.46  & 31.20 \\
    PVT~\cite{pvt} & PVT-T & Vanilla MLP   & 14.56 & 12.84 & 70.60 & 32.85 \\
    PVT~\cite{pvt} & PVT-T & DMLPv1   &  13.11  &  13.10  &  71.75  & 35.18~\gbf{+3.98} \\ 
    \rowcolor{gray!15} Trans4PASS & PVT-T$\dagger$ & DMLPv1+DPE  & 13.18 & 13.10 & 69.62 & 36.50~\gbf{+5.30} \\ \hline
    SegFormer~\cite{segformer} & MiT-B1   & Vanilla MLP & 13.27 & 13.66 & 74.93  & 39.02 \\
    SegFormer~\cite{segformer} & MiT-B1   & FPN    & 9.88 & 13.58 & 73.96 & 41.14 \\
    SegFormer~\cite{segformer} & MiT-B1   & DMLPv1    &   11.82    &   13.92 &  73.10  & 45.14~\gbf{+6.12} \\
    \rowcolor{gray!15} Trans4PASS & MiT-B1$\dagger$ & DMLPv1 & 12.02 & 13.93 & 72.49 & \textbf{45.89}~\gbf{+6.87} \\ \midrule
    \multicolumn{7}{@{}p{\columnwidth}@{}}{\textit{\textbf{(3) Compare token mixing structures: }}} \\ \midrule
    Trans4PASS+ & MiT-B1$\dagger$ & {PoolFormer~\cite{yu2021metaformer}} & 9.47& 13.47& 70.52& 43.18 \\
    Trans4PASS+ & MiT-B1$\dagger$ & {FAN~\cite{zhou2022fan}} & 10.96& 13.81 & 71.15 &42.54 \\
    Trans4PASS+ & MiT-B1$\dagger$ & {PoolFormer~\cite{yu2021metaformer}+FAN~\cite{zhou2022fan}} & 10.96& 13.81& 72.21&45.97 \\
    Trans4PASS+ & MiT-B1$\ddag$ & {PoolFormer~\cite{yu2021metaformer}+FAN~\cite{zhou2022fan}} & 10.96& 13.81& 67.24& 47.69 \\
    Trans4PASS+ & MiT-B1$\dagger$ & {DMLPv2 (PX)} & 10.22 & {13.60} & {72.62} & 46.66~\gbf{+7.64} \\
    Trans4PASS+ & MiT-B1$\dagger$ & {DMLPv2 (CX)} & 11.70& 13.95 & 72.51& 47.06~\gbf{+8.04} \\
    \rowcolor{gray!15} Trans4PASS+ & MiT-B1$\dagger$ & {DMLPv2 (PX+CX)} & 11.70& 13.95 & 73.44& \textbf{47.74}~\gbf{+8.72} \\
    \rowcolor{gray!15} Trans4PASS+ & MiT-B1$\ddag$ & {DMLPv2 (PX+CX)} & 11.70& 13.95 & 72.67& \textbf{50.23}~\gbf{+11.21}\\
    \bottomrule
\end{tabular}}
% \vskip -2ex
\label{tab:ablation_structure}
% \vskip -3ex
\end{table}
